On Turing dynamical systems and the Atiyah problem

Main theorems of the article concern the problem of M. Atiyah on possible values of l^2-Betti numbers. It is shown that all non-negative real numbers are l^2-Betti numbers, and that "many" (for example all non-negative algebraic) real numbers are l^2-Betti numbers of simply connected manifolds with respect to a free cocompact action. Also an explicit example is constructed which leads to a simply connected manifold with a transcendental l^2-Betti number with respect to an action of the threefold direct product of the lamplighter group Z/2 wr Z. The main new idea is embedding Turing machines into integral group rings. The main tool developed generalizes known techniques of spectral computations for certain random walk operators to arbitrary operators in groupoid rings of discrete measured groupoids.

==> preambula-cmd.tex <==
\newcommand\Spec{\operatorname{Spec}}
\newcommand\tr{\operatorname{tr}}
\newcommand\alg{\operatorname{alg}}
\newcommand\esup{\operatorname{ \text{ess sup} }}
\newcommand\fin{\operatorname{fin}}
\newcommand\Sym{\operatorname{Sym}}
\newcommand\Dom{\operatorname{Dom}}

\newcommand\st{\operatorname{St}}
\newcommand\schr{\operatorname{Schr}}
\newcommand\cay{\operatorname{Cay}}
\newcommand\diag{\operatorname{Diag}}

\newcommand\dimvn{\dim_\text{vN}}


\newcommand{\field}[1]{{\mathbb #1}}
\newcommand{\F}[1]{{\frak #1}}
\newcommand{\Zmod}[1]{\,\Z{/#1\Z}\,}
\newcommand{\cc}[1]{{\mathcal #1}}
\newcommand{\call}[1]{{\mathcal #1}}
\newcommand{\B}[1]{{\field #1}}
\newcommand{\define}[1]{{\textbf{\textit{#1}}}}

\newcommand{\bb}[1]{{\mathbb #1}}
\newcommand{\actson}{{\curvearrowright}}
\newcommand{\mapsinto}{{\hookrightarrow}}

%\newcommand{\bf}[1]{{\textbf #1}}


\newcommand\R{\mathbb R}
\newcommand\Q{\mathbb Q}
\newcommand\Z{\mathbb Z}
\newcommand\C{\mathbb C}
\newcommand\N{\mathbb N}

\newcommand{\wt}[1]{{\widetilde {#1}}}
\newcommand{\wh}[1]{{\widehat {#1}}}
\newcommand{\ce}{{\mathcal C}}

%Greek characters
\newcommand{\p}{{\partial}}
\newcommand{\al}{{\alpha}}
\newcommand{\Al}{{\Alpha}}
\newcommand{\be}{{\beta}}
\newcommand{\Be}{{\Beta}}
\newcommand{\Om}{{\Omega}}
\newcommand{\om}{{\omega}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\de}{{\delta}}
\newcommand{\De}{{\Delta}}
\newcommand{\ga}{{\gamma}}
\newcommand{\Ga}{{\Gamma}}
\newcommand{\io}{{\iota}}
\newcommand{\ka}{{\kappa}}
\newcommand{\la}{{\lambda}}
\newcommand{\La}{{\Lambda}}
\newcommand{\si}{{\sigma}}
\newcommand{\Si}{{\Sigma}}
\newcommand{\vfi}{{\varphi}}
\newcommand{\gf}{{\varphi}}

%ABBREVIATIONS
\newcommand{\Mo}{(M,\omega )}
\newcommand{\Wo}{(W,\omega_W )}
\newcommand{\No}{(N,\omega_N )}
\newcommand{\cp}{\B C\B P}
\newcommand\BS{\operatorname{BSymp}}
\newcommand\ES{\operatorname{ESymp}}
\newcommand\BD{\operatorname{BDiff}}
\newcommand\ED{\operatorname{EDiff}}
\newcommand\BH{\operatorname{BHam}}
\newcommand\EH{\operatorname{EHam}}
\newcommand\E{\operatorname{E}}
\newcommand\gl{\operatorname{GL}}
\newcommand\pgl{\operatorname{PGL}}
\newcommand\psl{\operatorname{PSL}}

\newcommand\Diff{\operatorname{Diff}}
\newcommand\Flux{\operatorname{Flux}}
\newcommand\Symp{\operatorname{Symp}}
\newcommand\Ham{\operatorname{Ham}}
\newcommand\eFlux{\operatorname{\widetilde{Flux}}}
\newcommand\Homeo{\operatorname{Homeo}}

\newcommand\Hom{\operatorname{Hom}}
\newcommand\End{\operatorname{End}}
\newcommand\Aut{\operatorname{Aut}}
\newcommand\Map{\operatorname{Map}}

\newcommand\Der{\operatorname{Der}}
\newcommand\Out{\operatorname{Out}}
\newcommand\vol{\operatorname{vol}}
\newcommand\sgn{\operatorname{sgn}}
\newcommand\hamel{\operatorname{Hamel}}
\newcommand\CAL{\operatorname{Cal}}
\newcommand\im{\operatorname{im}}
\def\Im{\operatorname{Im}}

\newcommand\Int{\operatorname{Int}}
\newcommand\sign{\operatorname{sign}}
\newcommand\id{\operatorname{Id}}
\newcommand\cat{\operatorname{cat}}
\newcommand\wgt{\operatorname{wgt}}
\newcommand\grad{\operatorname{grad}\,}
\newcommand\sgrad{\operatorname{sgrad}}
\newcommand\crit{\operatorname{crit}}
\newcommand\Crit{\operatorname{Crit}}
\newcommand\Jac{\operatorname{Jac}}
\newcommand\supp{{\operatorname{supp}}}


%\newcommand{\la}{{\langle}}
%\newcommand{\ra}{{\rangle}}
%\newcommand{\ov}{{\overline}}

\newcommand{\wrt}{{\textit{w.r.t.} }}

\renewcommand{\thefootnote}{\fnsymbol{footnote}} 

==> preambula-pkg.tex <==
\usepackage{setspace}
%\onehalfspace
%\singlespace
%\setstretch{1.1}


%\usepackage{lscape}
\usepackage[centertags]{amsmath}
\usepackage{amsfonts}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{euscript}

%\usepackage{polski}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
%\usepackage[perpage]{footmisc}
\usepackage[american]{babel} %quotation marks

\usepackage[parskip=5pt,indention=5pt, scriptsize,tt]{caption}
\setlength{\captionmargin}{20pt}
\usepackage{subfig}
\usepackage{graphicx}

\usepackage{color}
\usepackage{epsfig}

\usepackage{url}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}


%\textwidth11.3in
%\textheight8in
%\voffset=-1.0in
%\hoffset=-0.8in


